InterLUDE: Interactions between Labeled and Unlabeled Data to Enhance Semi-Supervised Learning

Semi-supervised learning (SSL) seeks to enhance task performance by training on both labeled and unlabeled data. Mainstream SSL image classification methods mostly optimize a loss that additively combines a supervised classification objective with a regularization term derived solely from unlabeled data. This formulation neglects the potential for interaction between labeled and unlabeled images. In this paper, we introduce InterLUDE, a new approach to enhance SSL made of two parts that each benefit from labeled-unlabeled interaction. The first part, embedding fusion, interpolates between labeled and unlabeled embeddings to improve representation learning. The second part is a new loss, grounded in the principle of consistency regularization, that aims to minimize discrepancies in the model's predictions between labeled versus unlabeled inputs. Experiments on standard closed-set SSL benchmarks and a medical SSL task with an uncurated unlabeled set show clear benefits to our approach. On the STL-10 dataset with only 40 labels, InterLUDE achieves 3.2% error rate, while the best previous method reports 14.9%.

==> ablationdraft.tex <==
\begin{table*}[h]
% \resizebox{\textwidth}{!}{\begin{tabular}{c|ccc|cccccc}
% \hline
% Dataset   & \multicolumn{3}{c|}{CIFAR10} & \multicolumn{3}{c}{CIFAR100}          & \multicolumn{3}{c}{STL10} \\ \hline
% \#Label                         & 10      & 40      & 250      & 200 & 400 & \multicolumn{1}{c|}{2500} & 10     & 40     & 100     \\ \hline
% iMatch   &  31.90$\pm$4.1      &1.78$\pm$0.1        & 1.55$\pm$0.1 & 35.66$\pm$1.9      & 21.19$\pm$0.2    & \multicolumn{1}{c|}{13.39$\pm$0.1}  &27.49$\pm$6.6     &  3.14$\pm$0.2    &2.66$\pm$0.1     \\
% iMatch (w/o Embedding Fusion)   &  29.76$\pm$7.3      & 2.31$\pm$0.9        &1.64$\pm$0.1          &36.07$\pm$3.2     & 23.70$\pm$1.9    & \multicolumn{1}{c|}{ 13.88$\pm$0.3	}     &30.88$\pm$14.9      & 5.23$\pm$3.7     & 3.23$\pm$0.4       \\
% iMatch (w/o Relative Loss)      &  29.57$\pm$7.3         & 2.37$\pm$0.9          & 1.75$\pm$0.2         &  34.53$\pm$1.4   &  23.20$\pm$1.7   & \multicolumn{1}{c|}{14.07$\pm$0.6}     & 49.50$\pm$13.5       &3.75$\pm$0.4        & 3.36$\pm$0.3        \\ \hline
% iMatch+ & 12.29$\pm$ 7.4       & 1.55$\pm$0.1   & 1.49$\pm$0.1   &  23.60$\pm$1.2 &  16.32$\pm$0.3  & \multicolumn{1}{c|}{12.93$\pm$0.2}     & 25.83$\pm$9.9  &  4.56$\pm $0.9  &  3.23$\pm$0.3  \\
% iMatch+  (w/o Embedding Fusion) & 22.03$\pm$7.2        &    1.78$\pm$0.1     &   1.61$\pm$0.1       &   	23.38$\pm$1.8  &   	16.63$\pm$1.6  & \multicolumn{1}{c|}{14.00$\pm$0.6}     & 17.20$\pm$1.7       &   4.25$\pm$1.0    &   4.37$\pm$0.1      \\
% iMatch+ (w/o Relative Loss)    &20.07$\pm$8.0         &1.57$\pm$0.1   &  1.60$\pm$0.1      &23.63$\pm$0.9     & 16.33$\pm$0.8    & \multicolumn{1}{c|}{	13.15$\pm$0.1}     &19.14$\pm$3.6       &  4.71$\pm$1.0     &4.55$\pm$0.3         \\ \hline
% \end{tabular}}
% \caption{Ablation study on ViT backbone. All results are averaged with three random seeds and reported with a 95\% confidence interval. }
% \label{imatch_imatchplus_ablation}
% \end{table*}

==> backups/EntropyVersion/method.tex <==
%!!! XW comment: please modify the figure. 1. Remove the three dots between Weak and strong augmentation for unlabeled samples. 
% 2. Add several images instead of a single image for unlabeled samples. Several images can correspond to the three dots in embedding fusion.
\begin{figure*}[htb]
  \centering
 % \includegraphics[width=17cm]{figs/CentralFigure.pdf}
  \includegraphics[width=17cm]{figs/CentralFigure_20240110.pdf}

%  \vspace{2.0cm}
  \caption{iMatch Framework. The labeled and unlabeled data are individually subjected to both weak and strong augmentations. Subsequently, the backbone model extracts embeddings from these augmentations applied to the labeled and unlabeled samples. The process of embedding fusion involves employing effective interaction strategies to connect the latent embeddings derived from both labeled and unlabeled samples. The relative loss function is utilized to impose regularization on the relative differences observed in predictions resulting from the weak and strong augmentations applied to the unlabeled and labeled data samples. }
\label{methodfig}
\end{figure*}


There are two main components in the proposed iMatch algorithm, a theoretically grounded embedding fusion strategy and an innovative new loss. The two components work in synergy to effectively leverage training signals from the unlabeled data. The framework of iMatch is illustrated in Fig. \ref{methodfig}. We will explicitly introduce the components of the proposed framework in the following subsections. Alg.~\ref{alg:iMatch}
\input{algo_iMatch}

%use formulation to %summary the operation
\subsection{Embedding Fusion}

The performance of a deep learning task is closely related to its level of difficulty or complexity. In general, deep models tend to perform better as deep learning tasks become less challenging, and conversely, their performance tends to decrease as tasks become more difficult \cite{Li2022PN}. Fortunately, the complexity of a semi-supervised learning task $\mathcal{T}$ can be measured in terms of the information entropy $H({\mathcal{T}})$. Previous studies have highlighted the benefits of reducing information entropy in learning tasks across diverse domains \cite{Radnosrati2020PN, Yu2023PN, Jain2023PN}. In pursuit of this goal, we propose the embedding fusion strategy, which aims to effectively bridge the gap between unlabeled and labeled data while reducing the complexity inherent in semi-supervised learning tasks, thereby enhancing the overall model performance.

When provided with labeled and unlabeled data points $\boldsymbol{X}=\left \{ \mathcal{L} \cup  \mathcal{U}\right \}$, and the associated label set $ \hat{\boldsymbol{Y} }=\left \{ Y_{\mathcal{L}} \cup \hat{Y}_{\mathcal{U}} \right \} $, where $Y_{\mathcal{L}} $ is the true label of the labeled data, and $\hat{Y}_{\mathcal{U}}$ is the pseudo label for the unlabeled data. Note the quality of the pseudo label depends on the prediction ability of the trained model. 
Formally, the entropy of a semi-supervised learning task $\mathcal{T}$ can be formulated as \cite{Li2022PN}:
\begin{equation}
\label{ImageLevelcomplexity}
H(\mathcal{T};\boldsymbol{X})=H( \hat{\boldsymbol{Y}},\boldsymbol{X}) - H(\boldsymbol{X})
\end{equation}
The dataset $(\boldsymbol{X}, \hat{\boldsymbol{Y}})$ is considered as a collection derived from $\mathit{D}_{\mathcal{X},\mathcal{Y} }$, an unknown joint distribution encompassing data points and corresponding
% XW: I think the data points in this context can represent either raw images or their corresponding embeddings, akin to a signal in both the time domain and frequency domain.
labels from the feasible spaces $\mathcal{X}$ and $\mathcal{Y}$. Symbolically, this relationship can be denoted as $(\boldsymbol{X}, \hat{ \boldsymbol{Y}}) \sim \mathit{D} _{\mathcal{X},\mathcal{Y} }$ \cite{Shalev14book}. Consequently, the labels $\hat{ \boldsymbol{Y}}$ is considered a sample drawn from the labeled and unlabeled data points $\boldsymbol{X}$, represented as $\hat{\boldsymbol{Y}} \sim \mathit{D} _{\mathcal{Y}|\mathcal{X} } $.
Our proposed embedding fusion operates within the latent space, subsequently affecting the formulation of entropy for the semi-supervised learning task in the following manner \cite{Yu2023PN}:
\begin{equation} \label{LatentLevelEntropy}
    H(\mathcal{T}; (I+A)\boldsymbol{X})  = 
 H(\boldsymbol{\hat{Y}}_{e};(I+A)\boldsymbol{X}) - H(\boldsymbol{X}) 
\end{equation}
where $I$ is the identity matrix, and $A$ represents a specific embedding fusion strategy, realized by applying a linear transformation matrix to the embeddings. % The matrix A in this work can be learnable or predefined. 
The labels ${\hat{\boldsymbol{Y}}}_e$ is different from ${\hat{\boldsymbol{Y}}}$ because the pseudo label $(\hat{Y}_{\mathcal{U}})_e$ for the unlabeled data is generated by the model equipped with embedding fusion. Here, we designate the deep model without embedding fusion as $f_{\hat{\theta }} (\cdot )$, and denote the deep model with embedding fusion as $f_{{\hat{\theta }}_e} (\cdot )$, where the model parameters $\theta$ are trainable. Therefore, in the context of embedding fusion, the label set is denoted as ${\hat{\boldsymbol{Y}}}_e$, in which the pseudo label $(\hat{Y}_{\mathcal{U}})_e$ is generated by the model $f_{\hat{\theta }_e} (\mathcal{U} )$. Following the assumption in \cite{Yu2023PN}, the entropy change is then formulated as:
\begin{equation} \label{LinearNosieFormula}
 \bigtriangleup S(\mathcal{T},A\boldsymbol{X })
= H(\mathcal{T};\boldsymbol{X}) - H(\mathcal{T};(I+A)\boldsymbol{X})  
\end{equation}
To conduct a quantitative analysis of the entropy change arising from embedding fusion, upon substituting Formulas \ref{ImageLevelcomplexity} and \ref{LatentLevelEntropy} into \ref{LinearNosieFormula}, we will derive the following result:
\begin{equation} \label{EntropyChangeQuantative}
\resizebox{.99\hsize}{!}{ $
\begin{aligned}
 \bigtriangleup S(\mathcal{T})
 =&H(\hat{\boldsymbol{Y}};\boldsymbol{X}) - H(\boldsymbol{X}) -( H( {\hat{\boldsymbol{Y}}}_e;(I+A)\boldsymbol{X})- H(\boldsymbol{X} ))\\
=&H(\hat{\boldsymbol{Y}};\boldsymbol{X}) - H({\hat{\boldsymbol{Y}}}_e;(I+A)\boldsymbol{X})\\
=&H(\hat{\boldsymbol{Y}}|\boldsymbol{X})+H(\boldsymbol{X}) - \left [ H({\hat{\boldsymbol{Y}}}_e|(I+A)\boldsymbol{X})+H((I+A)\boldsymbol{X})\right  ]   \\
=&\frac{1}{2} \log \frac{|\boldsymbol{\Sigma}_{\boldsymbol{X}}||\boldsymbol{\Sigma_{\hat{Y}}}-\boldsymbol{\Sigma_{\hat{Y}X}}{\boldsymbol{\Sigma_{X}^{-1}}}\boldsymbol{\Sigma_{X\hat{Y}}}|}{|\boldsymbol{\Sigma}_{(I+A)\boldsymbol{X}}||\boldsymbol{\Sigma_{\hat{Y}_e}-\Sigma_{ {\hat{Y}}_e X}}\boldsymbol{\Sigma^{-1}_{X}}\boldsymbol{\Sigma_{X\hat{Y}_e}}|} \\
=&\frac{1}{2} \log \frac{ 1 }{|I+A|^{2}} + \frac{1}{2} \log \frac{|\boldsymbol{\Sigma_{\hat{Y}}}-\boldsymbol{\Sigma_{\hat{Y}X}}{\boldsymbol{\Sigma_{X}^{-1}}}\boldsymbol{\Sigma_{X\hat{Y}}}|}{|\boldsymbol{\Sigma_{\hat{Y}_e}-\Sigma_{ {\hat{Y}}_e X}}\boldsymbol{\Sigma^{-1}_{X}}\boldsymbol{\Sigma_{X\hat{Y}_e}}|}\\
=&-\log|I+A| +\mathcal{M}( \hat{\theta}, \hat{\theta}_e(A) )
\end{aligned}
$}
\end{equation}
\todo{Assumption: each y and x in Y and X follows normal distribution.}
where the $\boldsymbol{\Sigma}$ represents the covariance matrix. We use $\mathcal{M}( \hat{\theta}, \hat{\theta}_e(A) )$ to represent the second term, i.e., $\frac{1}{2} \log \frac{|\boldsymbol{\Sigma_{\hat{Y}}}-\boldsymbol{\Sigma_{\hat{Y}X}}{\boldsymbol{\Sigma_{X}^{-1}}}\boldsymbol{\Sigma_{X\hat{Y}}}|}{|\boldsymbol{\Sigma_{\hat{Y}_e}-\Sigma_{ {\hat{Y}}_e X}}\boldsymbol{\Sigma^{-1}_{X}}\boldsymbol{\Sigma_{X\hat{Y}_e}}|}$ in entropy change. The presence of the second term can be attributed to the disparity between the pseudo label and the true label. \textbf{Note:} In an ideal scenario, where the pseudo labels assigned to the unlabeled data match precisely with the true labels, the second term $\mathcal{M}( \hat{\theta}, \hat{\theta}_e(A) )$ would be equal to 0. 
where the $\boldsymbol{\Sigma}$ represents the covariance matrix. We use $\mathcal{M}( \hat{\theta}, \hat{\theta}_e(A) )$ to represent the second term, i.e., $\frac{1}{2} \log \frac{|\boldsymbol{\Sigma_{\hat{Y}}}-\boldsymbol{\Sigma_{\hat{Y}X}}{\boldsymbol{\Sigma_{X}^{-1}}}\boldsymbol{\Sigma_{X\hat{Y}}}|}{|\boldsymbol{\Sigma_{\hat{Y}_e}-\Sigma_{ {\hat{Y}}_e X}}\boldsymbol{\Sigma^{-1}_{X}}\boldsymbol{\Sigma_{X\hat{Y}_e}}|}$ in entropy change. The presence of the second term can be attributed to the disparity between the pseudo label and the true label. \textbf{Note:} In an ideal scenario, where the pseudo labels assigned to the unlabeled data match precisely with the true labels, the second term $\mathcal{M}( \hat{\theta}, \hat{\theta}_e(A) )$ would be equal to 0. 

The first component in Formula \ref{EntropyChangeQuantative} elucidates the impact of embedding fusion from the perspective of data points, including the labeled and unlabeled data. In contrast, the second component is rooted in the imperfect prediction of pseudo-labels for unlabeled data, demonstrating the combined influence of the embedding fusion strategy and deep model parameters on altering entropy. In pursuit of improved performance in semi-supervised learning tasks, our objective is to realize entropy reduction (i.e., making $ \bigtriangleup S(\mathcal{T}) > 0$ ). Consequently, in this paper, guided by Formula \ref{EntropyChangeQuantative}, we explore effective embedding fusion to achieve improved performance. Delving into the first term, one can find that the first term can be $+\infty $ as long as the determinant of $I+A$ equals $0$. However, it is neither reasonable nor feasible for $|I+A|$ to equal 0, as this would result in the annihilation of image information, given that $|I+A|\boldsymbol{X}$ would then become $\textbf{0}$. Therefore, to make the embedding fusion meaningful, there are constraints 
\begin{equation} 
\begin{split}
&s.t. \ rank(I+A)=k \\
&\ \quad  \left [ I+A\right ]_{ii} > \left [ I+A \right ]_{ij}, i \ne j \\
& \ \quad  \left \| \left [ I+A\right ]_{i}   \right \|_{1} = 1 
\end{split}
\end{equation}
where $k$ is the number of images in a mini-batch. The first constraint is the most important one that ensures that $I+A$ is full rank. The full rank requirement ensures that the embeddings of images will not be eliminated. The second constraint is to make the trained classifier get enough information about a specific image and correctly predict the corresponding label. For example, for an image $x_{1}$ perturbed by another image $x_{2}$, the classifier obtained dominant information from $x_{1}$ so that it can predict the label $y_{1}$. However, if the perturbed image $x_{2}$ is dominant, the classifier can hardly predict the correct label $y_{1}$ and is more likely to predict as $y_{2}$. The third constraint is to maintain the norm of latent representations. 

Although direct control over the second term is not feasible due to its dependence on model parameters and entanglement with the first term, we can directly optimize the first term, thereby indirectly impacting the second term, to realize entropy reduction. The key to determining the quality of the embedding fusion lies in the matrix of $A$. In this work, we adopt the circular shift \cite{zhang2020CS} as the embedding fusion strategy. Specifically, the embedding fusion strategy employed in the paper is depicted in Fig. \ref{embeddingfusion}. To fulfill the constraints and achieve entropy reduction, we employ a hyperparameter, denoted as $\alpha$, to regulate the fusion strength. For example, assuming the number of samples of labeled and unlabeled data in a mini-batch is $k$, then the strategy $A$ can be denoted as $\alpha * U_{i,j} - \alpha * I_{k\times k}$, where $U_{i,j}=\delta_{i+1,j} $, and $\delta_{i+1,j}$ is the Kronecker delta symbol. Typically, a higher embedding fusion strength can yield a larger value for the first term in Formula \ref{EntropyChangeQuantative} compared to that resulting from a lower fusion strength. 

% Nevertheless, this heightened fusion strength could potentially compromise the quality of pseudo-labels for unlabeled data, thereby causing the second term to decrease.

Detailed derivation of embedding fusion and in-depth analysis are included in the supplementary.

\subsection{Relative Consistency}
\label{RelativeLoss}
Denoted by 
$\omega(\cdot)$ and $\Omega(\cdot)$
 respectively as a predefined set of weak and strong augmentation operations, $\omega(\cdot)_{m}$ and $\Omega(\cdot)_{m}$ as a random sample from $\omega(\cdot)$ and $\Omega(\cdot)$.
For a labeled sample $x_{l}^{(i)} \in \mathcal{L}$, we generate a weakly augmented sample $x_{l}^{(i)w}$ and a strongly augmented sample $x_{l}^{(i)s}$ using $\omega(\cdot)_{m}$ and $\Omega(\cdot)_{m}$. For each unlabeled sample $x_{u}^{(j)} \in \mathcal{U}, j \in \{1,\ldots,\mu\}$, where $\mu$ is the ratio of unlabeled data batch size to labeled data batch size as in~\citep{sohn2020fixmatch}, we apply the \textit{same} weak and strong augmentation $\omega(\cdot)_{m}$ and $\Omega(\cdot)_{m}$ to obtain $x_{u}^{(j)w}$, and $x_{u}^{(j)s}$, $j\in\{1,\ldots,\mu\}$. The difference in augmentation $a(\cdot)_{m}$ and $A(\cdot)_{m}$ results in the difference in predictions for the same data.

The Relative Loss is designed based on the widely used consistency regularization principle. However, as noted in prior work~\citep{huang2023flatmatch}, most consistency-regularization based algorithms only applies ``instance-wise'' consistency (i.e., consistency on each sample with its own transformation), and most often only on the unlabeled data. In contrast, our relative loss is designed to regularize behaviors \emph{between} labeled and unlabeled samples.

Denote $p(y|x_{u}^{(j)w})$ and $p(y|x_{u}^{(j)s})$ as $q_{j}^w$  and $q_{j}^s$, $p_(y|x_{l}^{(i)w})$ and $p_(y|x_{l}^{(i)s})$ as $p_{i}^w$ and $p_{i}^s$.

We measure the difference as
\begin{align}
d_{x,m}^{\text{diff}} &= p_{i}^w - p_{i}^s, \label{eq:diff_labeled}\\
d_{u,m}^{\text{diff}} &= \frac{1}{\mu} \sum_{j=1}^{\mu}(q_{j}^w - q_{j}^w)\label{eq:diff_unlabeled}
\end{align}

% \begin{align}
% d_{x,m}^{\text{diff}} &= p(y|x_{i}^w) - p(y|x_{i}^s), \\
% d_{u,m}^{\text{diff}} &= \frac{1}{\mu} \sum_{j=1}^{\mu}p(y|u_{j}^w) - p(y|u_{j}^s)
% \end{align}

Our Relative Consistency aims to encourage the unlabeled data to mimic the behavior of the labeled data given the same set of augmentation. In doing so, we exploit the interaction between labeled and unlabeled data. To implement the Relative Consistency, we use L2 loss in this paper since it is bounded
~\citep{berthelot2019mixmatch}.
% and might cause less fluctuation to the training dynamics 
\begin{align}
\mathcal{L}_{rel}= \frac{1}{B}\sum_{i=1}^{B}\left\| d_{x,m}^{\text{diff}} - d_{u,m}^{\text{diff}} \right\|_2^2 \label{eq:loss_rel}
\end{align}
We use the same weak and strong augmentation as in ~\citep{sohn2020fixmatch}, which includes random flip and crop for the weak augmentation and RandAug~\citep{cubuk2020randaugment} for the strong augmentation. Since $d_{x,m}^{\text{diff}}$ is serving as the target for $d_{u,m}^{\text{diff}}$ to encourage model behavior on unlabeled data mimic that of on labeled data, a stop-gradient is applied on $d_{x,m}^{\text{diff}}$ as a standard practice in SSL works that favors convergence~\citep{berthelot2021adamatch}.

% % \begin{align}
% % \ell_{rel}(d_{x}, d_{u})
% % \end{align}
% \begin{align}
% \ell_{s}(p_{x}^{w}, y)
% \end{align}


\begin{figure}[htb]
  \centering
 \includegraphics[width=8 cm]{figs/InterLeave_shrink.pdf}
%  \vspace{2.0cm}
  \caption{Embedding Fusion aims to bridge the gap between labeled and unlabeled data by circularly combining their embeddings. This circular process enables the embeddings of labeled data to incorporate information from the unlabeled set, while simultaneously allowing the embeddings of unlabeled data to be influenced by those from the labeled set. We show that this approach is effective in reducing the entropy associated with semi-supervised learning tasks, consequently enhancing performance.}
\label{embeddingfusion}
\end{figure}



\subsection{Instance-wise Consistency}
The instance-wise consistency loss is based on FixMatch ~\citep{sohn2020fixmatch}, and has since been widely used by various following works as part of the final objectives ~\citep{huang2023flatmatch,wang2022freematch,zheng2022simmatch,zheng2023simmatchv2}. The regular instance-wise consistency can be written as

\begin{align}
\label{eq:Lu}
\mathcal{L}_u = \frac{1}{\mu B} \sum_{j=1}^{\mu B} \mathbf{1} (\max (q_{j}^w) > \tau) H(q_{j}^w, q_{j}^s)
\end{align}

Where scalar $\tau$ is the confidence threshold. We fix $\tau=0.95$ throughout; the same setting as in ~\citep{sohn2020fixmatch,zheng2022simmatch}. 

% $DA(\cdot)$
% stands for the distribution alignment strategy from~\citep{berthelot2019remixmatch} which balanced the pseudo-labels distribution. 

\subsection{iMatch}
Putting it together, our iMatch contains a standard cross-entropy loss based on the labeled samples, a common instance-wise consistency loss on the unlabeled sample and the newly proposed relative consistency loss.

Our final loss function can be written as: 
\begin{align}
\mathcal{L}_s &= -\frac{1}{B} \sum_{i=1}^{B} y_{i} \log p_{i}^w \label{eq:supervised_loss}\\
\mathcal{L} &= \mathcal{L}_{s} + \lambda_{u}\mathcal{L}_u + \lambda_{rel} \mathcal{L}_{rel}\label{eq:imatch_total_loss}
\end{align}

where $\lambda_{u}$ and $\lambda_{rel}$ are balancing factors that control the weights of the different losses.

% We use standard cross-entropy loss only on the weakly augmented labeled samples. Denote $p(y|x_{i}^w)$ as $p_{i}^w$
% Our final loss function can be written as: 
% \begin{align}
% \mathcal{L}_s &= -\frac{1}{B} \sum_{i=1}^{B} y_{i} \log p_{i}^w \\
% \mathcal{L} &= \mathcal{L}_{s} + \lambda_{u}\mathcal{L}_u + \lambda_{rel} \mathcal{L}_{rel}
% \end{align}

% where $\lambda_{u}$ and $\lambda_{rel}$ are balancing factors that control the weights of the different losses.

\subsection{iMatch+}
Note that FlatMatch~\citep{huang2023flatmatch} has utilized the Self-Adaptive Threshold (SAT) and Self-Adaptive Fairness (SAF) technique proposed in~\citep{wang2022freematch}, which are techniques that could be widely applicable to various methods (including ours). To fairly compare with FlatMatch, we incorporate these techniques into our iMatch, and termed the enhanced algorithm iMatch+. Even without using SAT and SAF, our iMatch outperform FlatMatch in many cases while being competitive in other cases. 

SAT aim to adjust the pseudo-label threshold by considering both the global(dataset-specific) threshold and local (class-specific) threshold at different time step, each estimated via the model's current learning status. Similar techniques such as Distribution Alignment (DA)~\citep{berthelot2019remixmatch} and its variant~\citep{berthelot2021adamatch} has been proposed and used by various SSL algorithms~\citep{li2021comatch,zheng2022simmatch}. 
\begin{align}
\tau_t(c) &= \frac{\tilde{p}_t(c)}{\max\{\tilde{p}_t(c) : c \in [C]\}} \cdot \tau_t,
\end{align}
where $\tau_{t}$ is the gloabl threshold at time $t$ and $\tilde{p}_t(c)$ is the local threshold for class $c$ at time $t$.
\begin{align}
\tau_t =
\begin{cases} 
\frac{1}{C}, & \text{if } t = 0,\\
\lambda \tau_{t-1} + (1 - \lambda) \frac{1}{\mu B}
\sum_{j=1}^{\mu B}
\max(q_{j}^{w}), & \text{otherwise},
\end{cases}
\end{align}

\begin{align}
\tilde{p}_t(c) = 
\begin{cases} 
\frac{1}{C}, & \text{if } t = 0,\\
\lambda \tilde{p}_{t-1}(c) + (1 - \lambda) \frac{1}{\mu B} \sum_{j=1}^{\mu B} q_{j}^{w}(c), & \text{otherwise},
\end{cases}
\end{align}

SAF is a regularization term that encourage diverse model predictions on unlabeled data.

\begin{align}
\mathcal{L}_{saf} &= -H \left[ \text{SumNorm} \left( \frac{\tilde{p}_t}{\tilde{h}_t} \right), \text{SumNorm} \left( \frac{\bar{p}}{\bar{h}} \right) \right]
\end{align}

where 
\begin{align}
\bar{p} &= \frac{1}{\mu B} \sum_{j=1}^{\mu B} \mathbf{1} (\max (q_{j}^w) \geq \tau_t (\arg\max (q_{j}^w)) q_{j}^s, \\
\bar{h} &= \text{Hist}_{\mu B} \left( \mathbf{1} (\max (q_{j}^w) \geq \tau_t (\arg\max (q_{j}^w)) \hat{q_{j}^s} \right),
\\
\tilde{h}_t &= \lambda \tilde{h}_{t-1} + (1 - \lambda) \text{Hist}_{\mu B} (\hat{q_{j}^w})
\end{align}

$\text{SumNorm} = (\cdot) / \sum (\cdot)$. Hist means the histogram distribution. $\hat{q_{j}^w}$ and $\hat{q_{j}^s}$ are the one-hot encoding of $q_{j}^w$ and $q_{j}^s$. More details of the SAT and SAF should be refered to original paper~\citep{wang2022freematch}.

Incorporating SAT and SAF with iMatch, the loss function of iMatch+ can be written as: 
\begin{align}
\mathcal{L} &= \mathcal{L}_{s} + \lambda_{u}\mathcal{L}_{u} + \lambda_{rel} \mathcal{L}_{rel} + \lambda_{saf} \mathcal{L}_{saf}\label{eq:imatchplus_total_loss}
\end{align}


where $\tau_t(c)$ is used to replaced the fixed threshold $\tau$ in eq~\ref{eq:Lu}.

==> backups/EntropyVersion/method_20240113_xw.tex <==





%use formulation to %summary the operation
\section{Embedding Fusion}

The operations applied to latent representations are considered a promising technique for improving model robustness and performance. From manifold mixup to feature mixup to latent perturbation, numerous works demonstrate the effectiveness of the embedding level operations \cite{Verma2019ManifoldMixup, Pereira2021, Yaguchi2019MixFeat}. Remarkably, through a thoughtful and deliberate design of latent representation fusion strategy, NoisyNN has attained unparalleled accuracy in supervised learning tasks \cite{Yu2023PN}.
Inspired by these existing works, we propose the embedding fusion strategy, which aims to effectively bridge the gap between unlabeled and labeled representations in latent space, thereby enhancing the overall model performance.

Since our embedding fusion is realized via applying the linear transform to the embeddings, we innovatively propose an embedding fusion design matrix $A$ to represent the design space of the possible embedding fusion strategies. Therefore, the key to determining the quality of the embedding fusion lies in the matrix of $A$. In SSL scenarios, it is crucial to highlight three distinct types of interactions: those occurring among labeled data, interactions within unlabeled data, and interactions bridging labeled and unlabeled data. The differences in the design matrix $A$ result in the ways of these interactions. If we use the symbol $Z=\{Z_u \cup Z_l\}$ to denote the latent embeddings of unlabeled and labeled data, where $Z_u$ and $Z_l$ represent the embeddings of unlabeled and labeled images, respectively. The proposed embedding fusion takes place in the final layer of both the ResNet and ViT architectures. As the embedding fusion occurs deeper within the model, better performance can be anticipated \cite{Yu2023PN}. Our embedding fusion can be formulated as:
\begin{equation} \label{EmbeddingFusionFormula}
\begin{split}
&   Z^{'}=\left ( I+A \right )Z   \\
&s.t. \ rank(I+A)=k \\
&\ \quad  \left [ I+A \right ]_{ii} > \left [ I+A \right ]_{ij}, i \ne j \\
& \ \quad  \left \| \left [ I+A \right ]_{i}   \right \|_{1} = 1 
\end{split}
\end{equation}
where $k$ is the number of images in a mini-batch. The first constraint that ensures that $I+A$ is full rank. The full rank requirement ensures that none of the embeddings of images will be eliminated. The second constraint is to make the trained classifier get enough information about a specific image and correctly predict the corresponding label. For example, for an image $x_{1}$ perturbed by another image $x_{2}$, the classifier obtained dominant information from $x_{1}$ so that it can predict the label $y_{1}$. However, if the perturbed image $x_{2}$ is dominant, the classifier can hardly predict the correct label $y_{1}$ and is more likely to predict as $y_{2}$. The third constraint is to maintain the norm of latent representations. 

In this work, we adopt the circular shift \cite{zhang2020CS} as the embedding fusion strategy. Specifically, the embedding fusion strategy employed in the paper is depicted in Fig. \ref{embeddingfusion}. To fulfill the constraints and achieve entropy reduction, we employ a hyperparameter, denoted as $\alpha$, to regulate the fusion strength. For example, assuming the number of samples of labeled and unlabeled data in a mini-batch is $k$, then the strategy $A$ can be denoted as $\alpha * U_{i,j} - \alpha * I_{k\times k}$, where $U_{i,j}=\delta_{i+1,j} $, and $\delta_{i+1,j}$ is the Kronecker delta symbol. For easy understanding, the linear transformation of the embeddings have the form as:
\begin{equation}
\begin{split}
 I+A =& \begin{bmatrix}
 1 &  &  &  &\\
  & 1 &  & &\\
  &  & . & &\\
  &  &  & 1& \\
  &  &  & &1
\end{bmatrix} + \begin{bmatrix}
 -\alpha & \alpha  &  &  &\\
  & . & .&  &\\
  &  & . &. &\\
  &  &  & . & \alpha\\
\alpha  &  &  & &-\alpha
\end{bmatrix}  \\
 =&
\begin{bmatrix} 
1-\alpha &\alpha  &  &  &\\
  & . & . & &\\
  &  & . &. &\\
  &  &  & .& \alpha \\
\alpha  &  &  & &1-\alpha
\end{bmatrix}
\end{split}
\end{equation}

\begin{figure}[htb]
  \centering
 \includegraphics[width=8 cm]{figs/InterLeave_BatchVersion.pdf}
%  \vspace{2.0cm}
  \caption{Embedding Fusion aims to bridge the gap between labeled and unlabeled data by circularly combining their embeddings. This circular process enables the embeddings of labeled data to incorporate information from the unlabeled set, while simultaneously allowing the embeddings of unlabeled data to be influenced by those from the labeled set. }
\label{embeddingfusion}
\end{figure}

==> backups/EntropyVersion/related_work.tex <==
\subsection{Semi-supervised learning}

In typical semi-supervised image classification problem, we are given a labeled dataset $\mathcal{L}$ of image-label pairs $(x_{l}, y)$, and an unlabeled dataset $\mathcal{U}$ containing only images $x_{u}$ with $|\mathcal{U}| \gg |\mathcal{L}|$. Our goal is to train a neural network that maps each image to probability vector in the $C$-dimensional simplex  $\Delta^C$ representing a distribution over $C$ class labels, using both the labeled set $\mathcal{L}$ and unlabeled set $\mathcal{U}$. Various SSL paradigms have been proposed over the past decades~\citep{blum1998combining,min2020mutually, kingma2014semi,kumar2017semi,nalisnick2019hybrid,liu2019deep}. Here, we mainly focus on the current dominant paradigm that combines a supervised classification objective with
additional regularization term derived from unlabeled data, to which our approach belongs. 
More comprehensive reviews can be found in~\citet{zhuSemiSupervisedLearningLiterature2005,chapelle2009semi,van2020survey}. 


This paradigm trains a neural network classifier $f$ with weights $\theta$ by solving the optimization problem:
\begin{align} % Use \! to reduce whitespace between symbols
\min_{\theta} ~ \!
	\textstyle \sum_{x_{l},y \in \mathcal{D}^L} \!
		\ell^L( y, f_{\theta}(x_{l}) )	
	+ 
	\lambda \!
	\sum_{x_{u} \in \mathcal{D}^U} \!
		\ell^U(f_{\theta}(x_{u}))
	\label{eq:standard_ssl_objective}
\end{align}
Here $\ell^L$ is a standard supervised cross entropy loss often based \emph{solely} on the labeled set and $\ell^U$ is a method-specific unlabeled-set loss often based \emph{solely} on the unlabeled set. 

This paradigm has produced plenty SOTA algorithms~\citep{lee2013pseudo,laine2016temporal,miyato2018virtual,tarvainen2017mean,sohn2020fixmatch,xu2021dash,zhang2021flexmatch}, including the most recent work ~\citep{wang2022freematch, chen2023softmatch,huang2023flatmatch}.

Popular approaches under this paradigm include: \textit{Pseudo-labeling} that impute labels for unlabeled dat~\citep{lee2013pseudo,arazo2020pseudo,xie2020self,rizve2021defense,cascante2021curriculum}; \textit{Consistency regularization}~\citep{laine2016temporal,sajjadi2016regularization,tarvainen2017mean,miyato2018virtual} that enforce consistent model outputs of the same unlabeled data under different perturbation; 
\textit{Hybrid} approach~\citep{berthelot2019mixmatch,sohn2020fixmatch,wang2022freematch, huang2023flatmatch} that combines several techniques at the same time. While successful, these approaches often lacks a deeper interplay\footnote{Implicit interactions exist. For example from the learning dynamics when the two loss term are minimized together during training or from the batch normalization operation.}  between labeled and unlabeled data, which we argue is a key limitation preventing them to fully harness the potential of unlabeled data.

FixMatch~\citep{sohn2020fixmatch} is a representative hybrid method that combines pseudo-labeling with consistency regularization. Many recent efforts have primarily focused on enhancing FixMatch by adjusting its pseudo-labeling threshold~\citep{xu2021dash,zhang2021flexmatch,wang2022freematch,chen2023softmatch,li2023instant}. This line of work has led to notable stride in SSL performance. Instead of following this prevailing trend, this work investigates an effective way to derive new training signals from the interaction between labeled and unlabeled data, offering a novel perspective in SSL research.


% FixMatch~\citep{sohn2020fixmatch} is a representative hybrid approach that combines pseudo-labeling with consistency regularization. Due its empirical success, many recent state-of-the-art has recent year has seen significant interests in improving on FixMatch by modifying its pseudo-label process~\citep{li2023instant}. This line of work has produced numerous recent state-of-the-art methods~\citep{xu2021dash,berthelot2021adamatch,zhao2022dc,duan2022rda,wang2022freematch,guo2022class,huang2023flatmatch,chen2023softmatch,li2023instant}. In this paper, we take a detour of the current focus. Instead of focusing on modifying the pseudo-labeling process of FixMatch-based framework, we turn to exploring new training signals from the interplay of labeled and unlabeled data.

\subsection{SSL with direct labeled-unlabeled interaction}
MixMatch~\citep{berthelot2019mixmatch} use MixUp~\citep{zhang2017mixup} to transform randomly suffled samples (including both labeled and unlabeled) by linear interpolation, which introduce direct interaction between labeled and unlabeled data. 
% linearly interpolate the labeled images (and their labels) with unlabeled images (with their pseudo labels) using MixUp~\citep{zhang2017mixup} to produce the transformed labeled and unlabeled images (and their labels). A cross-entropy loss is then used on the transformed labeled data together with a mean squared error on the transformed unlabeled data.
However, the purpose of MixMatch is to ``unify dominant approaches to semi-supervised learning'', which is different from our main motivation of advocating interaction between labeled and unlabeled data. In SimMatch~\citep{zheng2022simmatch}, an additional loss term based on the unlabeled data is added to the standard ssl objective in eq ~\ref{eq:standard_ssl_objective}. This term exploit labeled-unlabeled interaction by enforcing the weak and strong augmented view of an unlabeled sample to have same similarity with the labeled embeddings. The connection is further entangled with the proposed  unfolding and aggregation operation. SimMatchV2~\citep{zheng2023simmatchv2} incorporate 4 different consistency losses from graph perspective. Specifically the ``Edge-Node Consistency'' uses the labeled samples to calibrate the pseudo-label of the weakly augmented unlabeled samples, introducing direct connection between labeled and unlabeled data. Compared to SimMatchV1/2, our approach is much simpler, does not require additional memory banks, and achieve better performance. 

Sharing similar spirit with ours, concurrent work FlatMatch~\citep{huang2023flatmatch} stress that labeled and unlabeled data are often disconnected during training in most existing SSL methods, as they only utilize ``instance-wise'' (i.e., consistency on each sample with its own transformation). FlatMatch seek connection between labeled and unlabeled data by utilizing Sharpness-Aware Minimization (SAM)~\citep{foret2020sharpness,kwon2021asam,liu2022towards,wu2020adversarial,zhang2022ga}. Specifically, it enforce the prediction on unlabeled sample to be close for regular model and the worst-case model, where the worst-case model is derived by adding perturbation to the regular model parameters that maximally increase the empirical risk on
labeled data. 
FlatMatch requires additional back-propagation to obtain the worst-case model, which doubles the computation complexity. This can be mitigated by an approximation strategy (FlatMatch-e). In contrast, our iMatch does not require additional back-propagation or approximation and achieves better and more stable performance (see Sec~\ref{Experiments}).

\subsection{Improving SSL with Embedding Fusion}
Recent studies emphasize the critical role of information entropy alterations within learning systems, unveiling their profound impact on the performance of designed frameworks \cite{Radnosrati2020PN, Li2022PN}.  Current research findings underscore the importance of reducing entropy as an effective approach to significantly enhance model performance across diverse learning tasks, such as image classification, domain adaptation, and language comprehension. Conversely, increasing information entropy could detrimentally affect model performances, potentially impeding the model's effectiveness in various applications \cite{Jain2023PN, Yu2023PN}. 

Currently, the mainstream approach to reducing entropy involves introducing diverse forms of noise into input images or latent representations. By designing appropriate strategies for adding noise into the input image or embedding procedures, the model has the potential to enhance its performance by decreasing entropy \cite{Zhang2023PN, Lin2023PN, Yu2023PN}. In SSL, entropy minimization has also been explored to improve model performance \cite {grandvalet2004semi,lee2013pseudo}, mainly by  encouraging the model to output confident predictions on unlabeled data.

Building upon existing research, this study presents an innovative embedding fusion approach operating within the latent space, aimed at reducing entropy and consequently enhancing model performance in semi-supervised learning (SSL) tasks. Theoretical proof shows the potential of our proposed embedding fusion to improve SSL learning, providing explicit and effective strategies for its implementation. The proposed embedding fusion integrates features from both labeled and unlabeled data, effectively bridging the divide between the two datasets and ensuring consistent regularization for both. Notably, it diverges from traditional consistency regularization methods that primarily focus on weak and strong augmentations of unlabeled data.

\subsection{Open-set SSL}
In classic SSL setting, labeled and unlabeled data are assumed to be sampled independently and identically from the same distribution. However, such assumption is often violated in real practice as unlabeled set are collected
automatically at scale for convenience, and thus uncurated ~\citep{oliver2018realistic,huang2023fix}. This more realistic scenario is often called ``open-set'' SSL ~\citep{yu2020multi,chen2020semi,guo2020safe,saito2021openmatch}.  

While our main focus in this paper is the classic SSL setting as in~\citep{zheng2023simmatchv2,wang2022freematch}, we also evaluate the performance of our iMatch on the open-set SSL benchmark proposed in ~\citep{huang2023fix}, and found that it perform well in the open-set ssl setting, even surpassing several recent strong robust SSL methods.


